The Summary Loop: Learning to Write Abstractive Summaries Without Examples

This work presents a new approach to unsupervised abstractive summarization based on maximizing a combination of coverage and fluency for a given length constraint. It introduces a novel method that encourages the inclusion of key terms from the original document into the summary: key terms are masked out of the original document and must be filled in by a coverage model using the current generated summary. A novel unsupervised training procedure leverages this coverage model along with a fluency model to generate and score summaries. When tested on popular news summarization datasets, the method outperforms previous unsupervised methods by more than 2 R-1 points, and approaches results of competitive supervised methods. Our model attains higher levels of abstraction with copied passages roughly two times shorter than prior work, and learns to compress and merge sentences without supervision.

==> original_intro.tex <==
% A summary is a brief statement or account of the main points of a longer, preceding document.
% Documents are summarized for multiple reasons, whether it is to attract the reader to read the original document (e.g. the headline of a blog post), or help determine the relevance of the document in a search.

% Two approaches exist to summarize documents: extractive and abstractive methods.
% In the extractive case, the summarizer (human or algorithmic) selects passages of the original document that are stitched into a summary. Abstractive summaries are not tied to the original document and are typically composed of words, and phrases from the original document as well as novel ones.
% In many domains requiring summarization (e.g. book summaries, research paper abstracts, news article summaries, tl;dr ...), human writers tend to be abstractive, by performing paraphrases, sentence compressions and merging, adding points of views.
% In the computational domain, both extractive and abstractive summarization algorithms have been proposed.

% An essential component to computational summarization is to define what a summary is, and propose a way to evaluate its quality.

% \textbf{What is a summary?} Most abstractive methods approach this question in a data-centric way. A dataset of pairs of documents and summaries are given as the gold standard. A summary is a text document that mimics ones in the dataset. For instance, summaries in the common CNN/DM dataset have an average of 3 sentences and 45 words. Therefore a model trained on CNN/DM produces summaries with an average of 3 sentences and 45 words. Given another dataset, the defining properties of the summary change. The data-centric approach is limiting in the case when data is scarce (low resource language or domain with less human-written summaries available).
% We attempt to produce the first summarization technique that is both dataset agnostic (unsupervised) and abstractive. In order to do this, we define what a summary is (see Section X), build automated scoring mechanism mirroring our definition, and directly optimize this score.

% \textbf{How to evaluate summary quality?} Evaluation of summary quality is an open problem. Ideally, summary quality should be based on its usefulness to a reader in a specific scenario. Because usefulness is subjective, the three most common evaluation methods abstract it away. The first method, human rating, asks human readers to rate summary properties such as informativeness, relevance, fluency and coherence on a scale. Two summarization methods can then be compared on each summary property evaluated, or on the overall average. Previous work has attempted to standardize human rating evaluation, however this remains challenging. In human ranking, the human reader is given a document and two summaries (a duel), and asked to make a choice of preference. The reader is given some guidelines as to what should be considered in the decision. A system is then considered better than another if it wins a majority of the duels. Finally, ROUGE score, is a fully automatic metric that computes summary quality based on n-gram overlap with target summaries. Even though it is shown to correlate with human assessments, ROUGE score has limitations. Paulus et al. trained a summarizing model that directly optimizes for high ROUGE score, and produced summaries that achieve very high ROUGE score, while being judged to be of low quality by human readers, due to their poor fluency (i.e. they do not contain full sentences).
% We propose to push Paulus' experiment a step further: we attempt to build a more comprehensive scoring mechanism for summaries following our definition and optimize this score in the same way.
Summarization, or the task to condense a document's main points into a smaller text document, appears in many textual domains, such as news headlines, research paper abstracts, Reddit TL/DRs or book back covers. These summaries serve different objectives, such as deliver the main piece of information, help a user decide whether to buy a product, or decide whether a document is relevant in a search.

Because of this diversity, giving an exact definition for the qualities of a summary is difficult, and most computational methods have taken a \textit{data-centric} approach to summarization. In the data-centric (or supervised) framework, a dataset (i.e. document-summary pairs) are given as the gold standard. A good summary is one that mimics summaries in the dataset. For instance, summaries in the common CNN/DM dataset have an average of 3 sentences and 45 words. Therefore a model trained on CNN/DM produces summaries with an average of 3 sentences and 45 words. Given another dataset, the defining properties of the summary change. The data-centric approach to summarization is limiting, as in some cases, data is rare or non-existent (low resource language or domain with less human-written summaries available).

In this paper we build an abstractive summarization method that does not rely on a dataset (i.e. it is unsupervised). We propose a definition for the qualities of a summary, and build the \textit{Summary Game} around this definition which we use to train a summarizer model with Reinforcement Learning. The models trained through this procedure achieve ROUGE performance within a few points of competitive supervised algorithms  on common news Summarization datasets (CNN/DM and Newsroom).

Our proposed definition for a Summary is the following:
\begin{quote}
    \centering
    ``A summary is a \underline{brief}, \underline{fluent} text that \underline{covers} the main points of an original document.''
\end{quote}

Brevity, fluency and coverage are the three pillars of a good summary. Under a length constraint, a quality summary should contain as much information about the original document while remaining in coherent English.
Section~\ref{section:summary_game} introduces the Summary game, which takes into account each pillar. However, we first demystify our approach to coverage through a motivating example.

\textbf{Motivation behind coverage.}
A relevant summary can be used to answer questions about the original document. For example, in Figure~\ref{fig:coverage_example}, either summary can be used to answer ``What country is this story about?'' or ``How many summits are getting cancelled?''. However, Summary 2 can be used to answer questions that Summary 1 cannot, such as "What are the names of the two summits?", or "Why were the summits cancelled?". We argue that if more questions can be answered with Summary 2 than Summary 1, Summary 2 covers the original document better than Summary 1.

Measuring coverage in this way is problematic however, as we do not have a way to generate comprehensive lists of questions about a document, or an easy way to determine whether a summary possesses the correct answer to a question. To solve this problem, we simplify the problem to using \textit{fill-in-the-blank} questions. Important words are masked out of the document and coverage is measured by seeing what fraction of the blanks can be filled with the information in the summary.

We operationalize the coverage idea, as well as the Fluency and Brevity pillars into a computational ``Summary Game'' in Section~\ref{section:summary_game}. In Section~\ref{section:training}, we show how to leverage the Summary Game to train a Summarization model without summary examples, and present results in Section~\ref{section:results}.
